MetaSensing: Intelligent Metasurface Assisted RF 3D Sensing by Deep Reinforcement Learning

Using RF signals for wireless sensing has gained increasing attention. However, due to the unwanted multi-path fading in uncontrollable radio environments, the accuracy of RF sensing is limited. Instead of passively adapting to the environment, in this paper, we consider the scenario where an intelligent metasurface is deployed for sensing the existence and locations of 3D objects. By programming its beamformer patterns, the metasurface can provide desirable propagation properties. However, achieving a high sensing accuracy is challenging, since it requires the joint optimization of the beamformer patterns and mapping of the received signals to the sensed outcome. To tackle this challenge, we formulate an optimization problem for minimizing the cross-entropy loss of the sensing outcome, and propose a deep reinforcement learning algorithm to jointly compute the optimal beamformer patterns and the mapping of the received signals. Simulation results verify the effectiveness of the proposed algorithm and show how the sizes of the metasurface and the target space influence the sensing accuracy.

==> sections/discussion.tex <==
%%%%%%%%%%
\section{Discussions}
%%%%%%%%%%
\label{sec: discussion}

%* 想做没有做的实验
%    * 扩展到大范围的实验
%    * 更多可控的超平面单元对于性能的提升效果
%    * 极限的成像距离

This paper designs and implements a prototype RIS-based RF-sensing system, HoloSketch, which can obtain semantic labeled point clouds for human and objects.
However, making this system complete requires additional technical challenges to be addressed.

%\parhead{Larger-space scenario}:
%The target space in this paper is confined within a small region.
%To extend HoloSketch and make it functioning well in large-scale space, the SNR of the received signals needs to be high enough to obtain accurate measurement.
%However, since the reflection on the RIS and objects results in the signal attenuation, it is challenging to ensure the sufficient received signal power at the receiver.
%To handle this issue, more sophisticated Tx and Rx antennas or LNAs with higher gain need to be adopted.


\parhead{Higher resolution:}
In this paper, the target space is divided into $0.4\times 0.2\times 0.2$ m$^3$ cubic regions, i.e., space blocks, which limits the resolution.
Increasing the resolution of HoloSketch requires the target space to be finely divided.
As described in Section~\ref{sec: obtain H}, to obtain the measurement matrix, a metal patch needs to be placed in each space block.
Therefore, to increase the resolution of HoloSketch implies the size of the metal patch needs to be shrunk and the number of measurements needs to be increased.
% 此外，小金属片使接收到的反射信号较小，因此需要更高增益的天线或者LNA。（不过这个上面说过了这里再说有点重复）=

\parhead{Faster data collection:}
In the data collection phase, the RIS changes its configuration by $0.1$ second, and thus the data collection phase lasts for at least $K/10$ seconds.
As the human and objects need to be static during the data collection phase, a long data collection phase due to large $K$ requires more efforts of ensuring them stay still when deploying HoloSketch.
To speed up the data collection procedure, we can adopt more advanced switching circuits and FPGA to shorten the time for changing the configurations of RIS.

\endinput

==> sections/implementation.tex <==
%%%%%%%%%%%%%%%%%
\section{Implementation}
%%%%%%%%%%%%%%%%%
\label{sec: system implementation}

\begin{figure}[!t]
	\center{\includegraphics[width=0.9\linewidth]{figures/implementation/ris_ctrl_circuit}}
	\vspace{-1em}
		\setlength{\belowcaptionskip}{-1.em}   %调整图片标题与下文距离
	\caption{Diagram of RIS control circuit.}
	\label{fig: RIS control circuit}
\end{figure}

%=================================
\subsection{Building the RIS}
%=================================
As shown in Fig.~\ref{fig: RIS control circuit}, the RIS is with the size of $69\times 69\times 0.52$ cm$^3$ and is composed of $16$ independently controllable groups which are tightly paved in squares.
Each group contains $12*12 = 144$ RIS elements arranged in a two-dimensional array, and thus the total number of RIS elements is $2304$.

Each RIS element has the size of $1.5\times 1.5 \times 0.52$ cm$^3$ and is composed of $4$ rectangle copper patches printed on a dielectric substrate~(Rogers 3010) with a dielectric constant of $10.2$ and $3$ PIN diodes~(BAR 65-02L).
Any two adjacent copper patches are connected by a PIN diode, and each PIN diode has two operation states, i.e., ON and OFF, which are controlled by applied bias voltages on the via holes.
When the applied bias voltage is $1.2$ V~(or $0$ V), the PIN diode is at the ON~(or OFF) state.

As there are $3$ PIN diodes in an RIS element, the total number of possible states of an RIS element is $8$.
We simulate the $S_{21}$ parameters, i.e., the \emph{forward transmission gain}, of the RIS element in different states for normal-direction incident RF signals in CST software, Microwave Studio, Transient Simulation Package~\cite{Hirtenfelder2007Effective}. 
%Table~\ref{table: S21 at 4 states} provides the amplitudes and angles of $S_{21}$ of an RIS element in $4$ of $8$ states for incident sinusoidal signals with frequency $3.2$~GHz.
We pick these four states with a phase shift interval equaling to $\pi/2$ as the \emph{available state set} $\mathcal S_a$, i.e., $\mathcal S_a = \{\hat{s}_1,\hat{s}_2,\hat{s}_3,\hat{s}_4\}$.
The four selected states have the phase values equaling to $\pi/4$, $3\pi/4$, $5\pi/4$ and $7\pi/4$, respectively.


As described in Section~\ref{ssec: ris model}, the RIS elements within the same group are in the same state.
The states of the $16$ groups are controlled by the RIS control circuit, which contains a direct current power supply, multiple voltage-stabilizing modules~(LM2596), $16$ digital switch circuit~(MAX4783), and a field-programmable gate array~(FPGA)~(ALTERA AX301).
The DC power supply is connected to the voltage-stabilizing modules, and the input voltage to the voltage-stabilizing modules is about $6$~V.
The voltage-stabilizing modules stabilize the input voltage and reduce it to a $1.2$ V output level. 
The digital switch circuits are single-pole double-throw and control whether the PIN diodes of RIS elements are connecting to the ground, i.e., $0$ V level, or to the $1.2$ V output of the voltage-stabilizing modules.

\begin{figure}[!t] % Example image
	\center{\includegraphics[width=0.9\linewidth]{./figures/implementation/scheme.pdf}}
	\vspace{-1.em}
	\setlength{\belowcaptionskip}{-1.2em}   %调整图片标题与下文距离
	\caption{Components of the transceiver module.}
	\label{fig: transceiver}
\end{figure}


%==========================================
\subsection{Building the Transceiver Module}
%==========================================
As shown in Fig.~\ref{fig: transceiver}, we build the RF transceiver module in HoloSketch by using the following components.

\parhead{(1) USRP devices}: We implement the Tx and Rx based on two~USRPs~(LW-N210), which are capable of converting baseband signals to RF signals, and vise versa.
The USRP is composed of the hardwares, including the RF modulation/demodulation circuits and baseband processing units, and can be controlled by using the GNU packet in Python~\cite{blossom2004gnu}.

\parhead{(2) Low-noise amplifiers~(LNAs)}: Since the RF signals need to be reflected twice~(on RIS and on objects) before reaching the Rx antenna, they suffer from large attenuation in signal strength, which results in low SNR and degrades the measurement accuracy.
To handle this issue, two LNA~(ZX60-43-S+) connect the Tx/Rx USRP and the Tx/Rx antenna and amplify the transmitted/received RF signals by about $15$ dB.

\parhead{(3) Tx and Rx antennas}: The Tx antenna is a directional double-ridged horn antenna~(LB-800), and the Rx antenna an omni-directional vertical antenna~(HT3500LC). 
The polarization of both the Tx and Rx antennas is linear and vertical to the ground.

\parhead{(4) Signal synchronizer}: For the Rx USRP to obtain the relative phases and amplitudes of the received signals with respect to the transmitted signals of the Tx USRP, we employ a signal source~(DG4202) to synchronize the frequency and phase of the Tx and Rx USRPs. The signal source provides the reference clock signal and the pulses-per-second~(PPS) signal to the USRPs, which ensures the modulation and demodulation of the USRPs to be coherent. 

\parhead{(5) Ethernet switch}: The Ethernet switch connects the USRPs and a sever forming a local Ethernet, where the controlling signals and received signals are exchanged.

\parhead{(6) Sever}: The sever controls the two USRPs by using the GNU packet in Python, extracts the measurement vectors from the received signals of the Rx USRP, and performs point cloud extraction and semantic segmentation.

\endinput

==> sections/pcextraction.tex <==

%========================
\section{Point Clouds Extraction}
%========================
\label{Extraction}

%In this section, we describe the point clouds extraction module and the compressive sensing technique in HoloSketch.


%========================
\subsection{Measurement Matrix Construction}
%========================
\label{sec: obtain H}

To perform point cloud extraction, we need first to construct the accurate values of the measurement matrix given the optimized configuration matrix $\bm C^*$ obtained by solving~(P1), as mapping $\bm g$ in Appendix 1 does not take the influence of the environment into account.
% 得解释清楚我们为什么要这么做
%The process to construct $\bm H$ is illustrated in Fig.~\ref{}.
To be specific, we first assign a set of $M$ spatial positions, which is denoted by $\mathcal M = \{(x_m, y_m, z_m)|m\in[1,M]\}$.
Then, we position a metal patch at the center of each spatial position, and collect the measurement vectors using the protocol described in Section~\ref{ssec: operating protocol} with the RIS using optimized configuration matrix $\bm C^*$.
When the metal patch is at the $m$-th~($m\in[1,M]$) spatial position, the collected measurement vector is denoted as $\hat{\bm y}_{\bm C^*, m}$.
%Following that, we collect the measurement vector when no metal patch is placed, i.e., the measurement vector for the background reflection, which is denoted as $\bm y^B$. 这种方法下面好像不需要收集background信号，两个一减就可以了。
Then, we remove the metal patch and obtain the measurement vector accounting for the background scattering, which is denoted as $\bm y^B_{C^*}$.
Based on the superposition property of the wireless signals, the channel gain for the propagation channel reflected at the $m$-th space block can be obtained by 
\beq
\bm h_{m}^* = ({\hat{\bm y}_{\bm C^*, m} - \bm y^B_{C^*}})/{\eta^{M}_{m}},
\eeq
where $\eta^{M}_{m}$ is the reflection coefficient of the metal patch at the $m$-th space block towards the Rx antenna. 
Moreover, for normalization, we assume $\eta^{M}_{m} = 1$, and thus each element in obtained $\bm\eta$ indicates the reflection coefficient with respect to the metal patch at that spatial position. 

Then, the measurement matrix $\bm H^* \in \mathbb C^{K\times M}$ corresponding to $\bm C^*$ can be formed by $\bm H ^*= [\bm h_1^*,...\bm h_M^*]$.
We use $\bm H$ to extract point cloud of target objects.
Denote the collected measurement vector as $\bm y$, and then the following equation holds
\beq
\label{equ: practical compressive sensing}
\bm y - \bm y^B  = \bm H \tilde{\bm \eta} + \bm e,
\eeq
where $\bm \eta\in \mathbb C^M$ is the reflection coefficient vector of the pre-assigned spatial positions with respect to metal patches.
Then, with known $\bm y$, $\bm y^B$, and $\bm H$, we can extract the point cloud by solving~(\ref{equ: practical compressive sensing}) to obtain $\bm \eta$, i.e., the normalized reflection coefficients of the spatial positions.

%===========================
\subsection{Reconstruction of Reflection Coefficients}
%===========================
Based on the compressive sensing technique described in Section~\ref{ssec: pce from rf signals}, we can obtain $\hat{\eta}$ by solving the following $l_1$-norm minimization problem:
\begin{align}
\text{(P2)}~
\min_{{\bm \eta}\in\mathbb C^{M}} \quad &\|{\bm \eta}\|_1,\\
& \|\bm H^*{\bm \eta} - \bm y_{\bm C^*} + \bm y^B_{\bm C^*}\|_2 \leq \epsilon. \nonumber
\end{align}
Here, $\epsilon$ is the variance of noise $\bm e$ in~(\ref{equ: practical compressive sensing}).
As~(P2) can be recast as a \emph{second-order cone program} problem, it can be solved using standard convex optimization tools in~\cite{Boyd_CONVEX}.
 
% The result vector $\hat{\bm \eta}$ is used to generate the point cloud.
From $\bm \eta$, the generation of the point cloud, which is a set of feature vectors and denoted by $\mathcal P$, is described as follows.
Set $\mathcal P$ contains $M$ elements, and each element is a $5$-dimensional feature vector, which is composed of its position and the reconstructed normalized reflection coefficient of it, i.e.,
\beq
\bm p_m = \left(
x_m, y_m, z_m, 
\mathrm{Re}({\bm \eta}_{m}),\mathrm{Im}({\bm \eta}_{m})
\right),~\forall m\in[1,M].
\eeq
Here, the first three dimensions of $\bm p_m$ indicate the coordinates of the $m$-th space block center, and $\mathrm{Re}$ and $\mathrm{Im}$ denote the real and imaginary parts of complex values, respectively.
\endinput
